Evidence for the spin-0 nature of the Higgs boson using ATLAS data

Studies of the spin and parity quantum numbers of the Higgs boson are presented, based on proton-proton collision data collected by the ATLAS experiment at the LHC. The Standard Model spin-parity JP = 0+ hypothesis is compared with alternative hypotheses using the Higgs boson decays H->gamma gamma, H -> ZZ -> 4 leptons and H->WW -> l nu l nu, as well as the combination of these channels. The analysed dataset corresponds to an integrated luminosity of 20.7 fb-1 collected at a centre-of-mass energy of sqrt(s) = 8 TeV. For the H -> ZZ -> 4-lepton decay mode the dataset corresponding to an integrated luminosity of 4.6 fb-1 collected at sqrt(s) = 7 TeV is added. The data are compatible with the Standard Model JP = 0+ quantum numbers for the Higgs boson, whereas all alternative hypotheses studied in this letter, namely some specific JP = 0-; 1+; 1-; 2+ models, are excluded at confidence levels above 97.8%. This exclusion holds independently of the assumptions on the coupling strengths to the Standard Model particles and in the case of the JP = 2+ model, of the relative fractions of gluon-fusion and quark-antiquark production of the spin-2 particle. The data thus provide evidence for the spin-0 nature of the Higgs boson, with positive parity being strongly preferred.

==> HWWlvlvPaper_Defs.tex <==

\newcommand{\UPD}{**UPDATE** }
\newcommand{\hwwlumi}{5.8}
\newcommand{\metrel}{\ensuremath{E_{\rm T,rel}^{\rm miss}}}
\newcommand{\mT}{\ensuremath{m_{\rm T}}}
\newcommand{\pTll}{\ensuremath{p_{\rm T}^{\ell\ell}}}
\newcommand{\ptll}{\pTll}
\newcommand{\vpTll}{\ensuremath{{\bf p}_{\rm T}^{\ell\ell}}}
%\newcommand{\dphill}{\ensuremath{\Delta\phi_{\ell\ell}}\xspace}
%\newcommand{\DPhill}{\ensuremath{\Delta\phi_{\ell\ell}}\xspace}
\newcommand{\dR}{\ensuremath{\Delta R}}
\newcommand{\pTtot}{\ensuremath{{\bf p}_{\rm T}^{\rm tot}}\xspace}
\newcommand{\njets}{\ensuremath{N_{\rm jets}}}
%\newcommand{\lhood}{\ensuremath{{\cal L}}}
\newcommand{\lelm}{\ensuremath{H{\rightarrow\,}WW^{(\ast)}{\rightarrow\,}e \nu \mu \nu}}
\newcommand{\wwlnln}{\ensuremath{WW^{(\ast)}{\rightarrow\,}\ell\nu\ell\nu}}
%\newcommand{\ZeroJet}{\ensuremath{\,H\!+0\mbox{-jet}}}
\newcommand{\ZeroJet}{\mbox{0-jet}}
\newcommand{\OneJet}{\mbox{1-jet}}
\newcommand{\TwoJet}{\mbox{2-jet}}
%\newcommand{\Ztt}{\ensuremath{Z/\gamma^{\ast}\to\tau\tau}\xspace}
%\newcommand{\Wjets}{$W$+jets}
\newcommand{\Wg}{\ensuremath{W\gamma^{(\ast)}}}
\def\MPT{\ensuremath{p_{\mathrm{T}}^{\mathrm{miss}}}}
\def\MPTRel{\ensuremath{p_{\mathrm{T, Rel}}^{\mathrm{miss}}}}
\newcommand{\hwwmll}{\ensuremath{m_{\ell\ell}}}

\def\WWSFzerojet{\ensuremath{1.06 \pm 0.06}} 
\def\WWSFonejet{\ensuremath{0.99 \pm 0.15}}

\def\TopSFzerojet{\ensuremath{1.11 \pm  0.06}}
\def\TopSFonejet{\ensuremath{1.11 \pm  0.05}}
\def\TopSFtwojet{\ensuremath{1.01 \pm  0.26}}

\def\Minpzero{\ensuremath{6 \times 10^{-4}}}
\def\Minpzerosigma{\ensuremath{3.2}}

\def\Nompzero{\ensuremath{8 \times 10^{-4}}}
\def\Nompzerosigma{\ensuremath{3.1}}

\def\NompzeroExp{\ensuremath{0.05}}
\def\NompzerosigmaExp{\ensuremath{1.6}}

\def\NompzeroCut{\ensuremath{2 \times 10^{-3}}}
\def\NompzerosigmaCut{\ensuremath{3.0}}

\def\NompzeroExpCut{\ensuremath{0.07}}
\def\NompzerosigmaExpCut{\ensuremath{1.5}}

\def\Nommu{\ensuremath{2.1^{+0.8}_{-0.7}}}
\def\NommuNoError{\ensuremath{2.1}}

\def\NommuOld{\ensuremath{0.5 \pm 0.7}} %2011
\def\DiffMuNewOld{\ensuremath{1.5}} %compatibility of 2011 and 2012 mu

\def\MinpzeroComb{\ensuremath{3 \times 10^{-3}}}
\def\MinpzerosigmaComb{\ensuremath{2.8}}
% Z = ROOT::Math::gaussian_quantile(1 - p0, 1)

\def\NompzeroExpComb{\ensuremath{0.01}}
\def\NompzerosigmaExpComb{\ensuremath{2.3}}

\def\NommuComb{\ensuremath{1.4 \pm 0.5}}

\def\CLexplow{\ensuremath{129}}
%\def\CLexphigh{\ensuremath{100}}
\def\CLobslow{\ensuremath{145}}
%\def\CLobshigh{\ensuremath{100}}

\def\CLexplowComb{\ensuremath{124}}
%\def\CLexphigh{\ensuremath{100}}
\def\CLobslowComb{\ensuremath{137}}
%\def\CLobshigh{\ensuremath{100}}

\def\threesigmaregion{\ensuremath{110-130}}

\def\TrackMETCut{\ensuremath{30}}
\def\CaloMETCut{\ensuremath{45}}
\def\CaloMETCutem{\ensuremath{25}}
\def\VBFCaloMETCutem{\ensuremath{20}}
\def\IsoCutRange{0.12-0.20}
\def\IsoConeSize{\ensuremath{0.3}}
\def\JVFCut{\ensuremath{0.5}}
\def\btagWP{\ensuremath{85\%}}

\def\WWSRErrorZerojet{\ensuremath{13\%}}
\def\WWSRErrorOnejet{\ensuremath{42\%}}
\def\TopSRErrorZerojet{\ensuremath{17\%}}
\def\TopSRErrorOnejet{\ensuremath{36\%}}
\def\TopSRErrorTwojet{\ensuremath{70\%}}
\def\WjetsSRError{\ensuremath{50\%}}
\def\WjetsSRErrorEle{\ensuremath{40\%}}
\def\WjetsSRErrorMu{\ensuremath{60\%}}

% 2011 numbers
% \def\WWSRErrorZerojet{\ensuremath{9\%}}
% \def\WWSRErrorOnejet{\ensuremath{22\%}}







==> resultcommands.tex <==

\newcommand{\lowerExpNoGeV}{110}
\newcommand{\lowerExp}{\lowerExpNoGeV\,GeV}
\newcommand{\upperExpNoGeV}{582}
\newcommand{\upperExp}{\upperExpNoGeV\,GeV}

%lowerlowerObs-uperlowerObs and lowerObs to upperObs
\newcommand{\lowerlowerObsNoGeV}{111}
\newcommand{\lowerlowerObs}{\lowerlowerObsNoGeV\,GeV}

\newcommand{\upperlowerObsNoGeV}{122} % 121.8
\newcommand{\upperlowerObs}{\upperlowerObsNoGeV\,GeV}

\newcommand{\lowerObsNoGeV}{131}
\newcommand{\lowerObs}{\lowerObsNoGeV\,GeV}
\newcommand{\upperObsNoGeV}{559}
\newcommand{\upperObs}{\upperObsNoGeV\,GeV}

%\newcommand{\lowerIsland}{112.7\,GeV}
%\newcommand{\lowerIslandNoGeV}{112.7}
%\newcommand{\upperIsland}{115.5\,GeV}
%\newcommand{\lowerupperObs}{251\,GeV}
%\newcommand{\lowerupperObsNoGeV}{251}
%\newcommand{\upperupperObs}{468\,GeV}
\newcommand{\significance}{$6.0\,\sigma$}
\newcommand{\expectedsignificance}{$4.9\,\sigma$}
\newcommand{\significanceESS}{$5.9\,\sigma$}

\newcommand{\lowerlowernintynineobsNoGeV}{1xx}
\newcommand{\upperlowernintynineobsNoGeV}{1yy}
\newcommand{\lowernintynineobsNoGeV}{1xy}
\newcommand{\upernintynineobsNoGeV}{5xy}
\newcommand{\lowerlowernintynineobs}{\lowerlowernintynineobsNoGeV\,GeV}
\newcommand{\upperlowernintynineobs}{\upperlowernintynineobsNoGeV\,GeV}
\newcommand{\lowernintynineobs}{\lowernintynineobsNoGeV\,GeV}
\newcommand{\upernintynineobs}{\upernintynineobsNoGeV\,GeV}

\newcommand{\lowernintynineexpNoGeV}{yyy1}
\newcommand{\upernintynineexpNoGeV}{yyy2}
\newcommand{\lowernintynineexp}{\lowernintynineexpNoGeV\,GeV}
\newcommand{\upernintynineexp}{\upernintynineexpNoGeV\,GeV}

\newcommand{\masspeak}{126.0}
\newcommand{\massresult}{\masspeak\pm 0.6~\mathrm{GeV}}
\newcommand{\massresultStatSys}{\mbox{\ensuremath{\masspeak \; \pm 0.4 \;\textrm{(stat)} \; \pm 0.4\; \textrm{(sys)}~\mathrm{GeV}}}}
%  m = 126.04    +0.39 -0.37 (stat)    +0.43 -0.44 (sys) GeV


